Multimode amplitude squeezing through cascaded nonlinear optical processes

Multimode squeezed light is enticing for several applications, from squeezed frequency combs for spectroscopy to signal multiplexing in optical computing. To generate squeezing in multiple frequency modes, optical parametric oscillators have been vital in realizing multimode squeezed vacuum states through second-order nonlinear processes. However, most work has focused on generating multimode squeezed vacua and squeezing in mode superpositions (supermodes). Bright squeezing in multiple discrete frequency modes, if realized, could unlock novel applications in quantum-enhanced spectroscopy and optical quantum computing. Here, we show how $Q$ factor engineering of a multimode nonlinear cavity with cascaded three wave mixing processes creates strong, spectrally tunable single mode output amplitude noise squeezing over 10 dB below the shot noise limit. In addition, we demonstrate squeezing for multiple discrete frequency modes above threshold. This bright squeezing arises from enhancement of the (noiseless) nonlinear rate relative to decay rates in the system due to the cascaded generation of photons in a single idler "bath" mode. A natural consequence of the strong nonlinear coupling in our system is the creation of an effective cavity in the synthetic frequency dimension that sustains Bloch oscillations in the modal energy distribution. Bloch mode engineering could provide an opportunity to better control nonlinear energy flow in the synthetic frequency dimension, with exciting applications in quantum random walks and topological photonics. Lastly, we show evidence of long-range correlations in amplitude noise between discrete frequency modes, pointing towards the potential of long-range entanglement in a synthetic frequency dimension.

==> preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
